ROA-Based Subharmonic Injection Locking for Oscillator-Based Ising Machines

This paper introduces on-chip integrated rotary traveling wave oscillators (RTWOs) organized into rotary oscillator array (ROA) bricks as an external perturbation to induce subharmonic injection locking (SHIL) in oscillator-based Ising machines (OIMs). The implementation of SHILs on chip is challenging, as the frequency of SHILs must be multiples of the operating frequency of the OIM nodes, with on-chip variations affecting the phase, degrading the SHIL process. This impedes the scaling of OIM implementations, regardless of the topology of Ising nodes, coupling or graph mapping mechanisms. The ROA brick topology implementation of RTWOs generates high frequency signals that are shown to provide a stable 2.31 GHz SHIL signal under process, voltage, and temperature (PVT) variations. Under PVT variations, distributed ring oscillator-based SHILs (ROSC-SHIL) fail to perform injection locking while the proposed ROA brick-based SHIL (ROA-SHIL) preserve 93% to 97% accuracy (the same accuracy of an ideal SHIL signal) in the OIM solutions of a sample 324-node max-cut problem. The driving strength and floorplan of the ROA brick are also shown to be amenable for scaling with an energy-to-solution impact of 2.49 nJ for the proposed ROA-SHIL.

==> circuitikz_diagrams/big_node_diagram.tex <==
  \newcounter{node}
  \newcounter{angle}
  \setcounter{node}{0}
  \setcounter{angle}{0}
  \newcommand{\maxx}{10}
  \newcommand{\maxy}{8}
  \foreach \y in {0,1,...,\maxy}
  {
    \foreach \x in {0,1,...,\maxx}
    {
      \ifnum\value{angle}=0
        \setcounter{angle}{180}
      \else
        \setcounter{angle}{0}
      \fi
      \node[circle, draw, ultra thick, minimum size=0.5cm, anchor=center](\thenode) at (\x,\y) {};

      \addtocounter{node}{1}
    }
  }

  \setcounter{node}{0}
  \foreach \y in {0,1,...,\maxy}
  {
    \foreach \x in {0,1,...,\maxx}
    {
      \pgfmathtruncatemacro{\trn}{\thenode+1+(\maxx+1)}
      \pgfmathtruncatemacro{\brn}{\thenode+1-(\maxx+1)}
      \pgfmathtruncatemacro{\bn}{\thenode-(\maxx+1)}
      \pgfmathtruncatemacro{\rn}{\thenode+1}
      % Draw down if y good
      \ifnum\y>0
        \draw (\thenode) -- (\bn);
        % Draw diagonal if both good
        \ifnum\x<\maxx
          \draw (\thenode) -- (\brn);
        \fi
      \fi

      % Draw right if x good
      \ifnum\x<\maxx
        \draw (\thenode) -- (\rn);
        % Draw top-right if both good
        \ifnum\y<\maxy
          \draw (\thenode) -- (\trn);
        \fi
      \fi

      \addtocounter{node}{1}
    }
  }
\node[draw, tdplot_main_coords] {} (current bounding box.north east) -- (current bounding box.north west) -- (current bounding box.south west) -- (current bounding box.south east) -- cycle;


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "paper"
%%% End:


==> circuitikz_diagrams/roa_brick.tex <==
%\documentclass[tikz,convert={outfile=rtwo_nodes.svg}]{standalone}
%\usepackage[siunitx, RPvoltages]{circuitikz}
%\graphicspath{{figures/}}
%
%\newsavebox{\rtwo}
%\sbox{\rtwo}{
  \tikzset{
    pics/rtwo/.style n args={3}{
      code={
        \draw[line width=0.1] (0,0)
         -- ++(6,0) node(br_out){}
         -- ++(0,6) node(tr_out){}
         -- ++(-5,0) node(tl_out){}
         -- ++(0,-5) node(bl_in){}
         -- ++(4,0)  node(br_in){}
         -- ++(0,4)  node(tr_in){}
         -- ++(-5,0) node(tl_in){}
         -- ++(0,-5) node(bl_out){};
        \ifnum#3=1
        \draw[-{Latex[scale=0.4]}] #2 node[squarepole, scale=5]{}
          -- ++(0,3) node[above, scale=4] {1};
        \fi

        \ifnum#3=-1
        \draw[-{Latex[scale=0.4]}] #2 node[squarepole, scale=5]{}
          -- ++(0,-3) node[below, scale=4] {1};
        \fi

        \node[scale=4] at (3,3) {#1};
        %\draw (tr_out) -- (bl_out);
      }
    }
  }
  %\begin{circuitikz}[scale = 0.5, transform shape]
  %  \pic{b2b_inv};
  %\end{circuitikz}
  %\pic[scale=0.1, every node/.style={scale=0.5}] (rtwo1) at (0,0) {rtwo={R1}{(4.5,9)}};
  \pic (rtwo1) at (7,9) {rtwo={R1}{(3,5)}{1}};
  \pic (rtwo2) at (14,16) {rtwo={R2}{(3,0)}{-1}};
  \pic (rtwo3) at (21,9) {rtwo={R3}{(3,6)}{1}};
  \pic (rtwo4) at (14,2) {rtwo={R4}{(3,1)}{-1}};
  % R1 to R2
  \draw[densely dotted]
        (rtwo1tr_out.center) node[circ, scale=3]{}
     -| (rtwo2bl_in.center) node[circ, scale=3]{};
  \draw[densely dashed]
        (rtwo1tr_in.center) node[circ, scale=3]{}
     |- (rtwo2bl_out.center) node[circ, scale=3]{};

  % R2 to R3
  \draw[densely dotted]
        (rtwo2br_out.center) node[circ, scale=3]{}
     |- (rtwo3tl_in.center) node[circ, scale=3]{};
  \draw[densely dashed]
        (rtwo2br_in.center) node[circ, scale=3]{}
     -| (rtwo3tl_out.center) node[circ, scale=3]{};

  % R3 to R4
  \draw[densely dotted]
        (rtwo3bl_out.center) node[circ, scale=3]{}
     -| (rtwo4tr_in.center) node[circ, scale=3]{};
  \draw[densely dashed]
        (rtwo3bl_in.center) node[circ, scale=3]{}
     |- (rtwo4tr_out.center) node[circ, scale=3]{};

  % R4 to R1
  \draw[densely dotted]
        (rtwo4tl_out.center) node[circ, scale=3]{}
     |- (rtwo1br_in.center) node[circ, scale=3]{};
  \draw[densely dashed]
        (rtwo4tl_in.center) node[circ, scale=3]{}
     -| (rtwo1br_out.center) node[circ, scale=3]{};

  %\begin{tikzpicture}
  %  \node {\includegraphics[width=7.5cm]{rtwo_layout.png}};
  %\end{tikzpicture}
%}


%%% Local Variables:
%%% mode: LaTeX
%%% TeX-master: t
%%% End:

